Full-Body Awareness from Partial Observations

There has been great progress in human 3D mesh recovery and great interest in learning about the world from consumer video data. Unfortunately current methods for 3D human mesh recovery work rather poorly on consumer video data, since on the Internet, unusual camera viewpoints and aggressive truncations are the norm rather than a rarity. We study this problem and make a number of contributions to address it: (i) we propose a simple but highly effective self-training framework that adapts human 3D mesh recovery systems to consumer videos and demonstrate its application to two recent systems; (ii) we introduce evaluation protocols and keypoint annotations for 13K frames across four consumer video datasets for studying this task, including evaluations on out-of-image keypoints; and (iii) we show that our method substantially improves PCK and human-subject judgments compared to baselines, both on test videos from the dataset it was trained on, as well as on three other datasets without further adaptation. Project website: https://crockwell.github.io/partial_humans

==> tables/new_ab_vlog.tex <==
\begin{table}[t]
\centering
    \caption{A/B testing on VLOG. For each entry we report how frequently the row wins/ties/loses to the column. For example, 
    the outputs of our full method is preferred over the outputs of the base method 62.7\% of the time, with 22.8\% of the entries
    rated as a tie.}
    \begin{tabular}{l@{~~~~}c@{~~~~}c} \toprule
    Method & Base & Crops \\ \midrule
$\downarrow$\,$>$/$=$/$<$\,$\rightarrow$  
    & $>$~/~$=$~/~$<$ 
    & $>$~/~$=$~/~$<$ 
    \\
Crops 
    & 53.3/27.5/19.2
    & -
    \\
Full
    & 62.7/22.8/14.5
    & 45.1/42.6/12.3
\\ \bottomrule
\end{tabular}
\end{table}



\begin{comment}
\begin{table}[t]
\centering
    \begin{tabular}{l|ccc|ccc|}

    Method & \multicolumn{3}{c|}{Base} & \multicolumn{3}{c|}{Crops} 
    \\
    $\downarrow > \rightarrow$ 
    & $>$ 
    & $=$ 
    & $<$ 
    & $>$ 
    & $=$ 
    & $<$ 
    \\
    A & B & C & D & E & F & G
\end{tabular}

\end{table}

\begin{table}[t]
\centering
\caption{A/B Test on VLOG}
\resizebox{\ifdim\width>\columnwidth \columnwidth \else \width \fi}{!}{
    \begin{tabular}{l@{~~} @{~~}|cc|@{~~} @{~~}|cc|@{~~} @{~~}|cc|@{~~}c@{~~}|cc|@{~~}@{~~}|cc|@{~~}@{~~}|cc|} \toprule
 &      \multicolumn{6}{c}{HMR \cite{KanazawaHMR17}} & ~ &
        \multicolumn{6}{c}{CMR \cite{Kolotouros19}} 
\\
Method & 
\multicolumn{2}{c}{$>$} & 
\multicolumn{2}{c}{$<$} & 
\multicolumn{2}{c}{$=$} & &
\multicolumn{2}{c}{$>$} & 
\multicolumn{2}{c}{$<$} & 
\multicolumn{2}{c}{$=$} 
\\
$\downarrow \ge \rightarrow$
        & Base  & Crop 
        & Base  & Crop 
        & Base  & Crop &
        & Base  & Crop 
        & Base  & Crop 
        & Base  & Crop 
        \\ 
        \midrule
Crop    
        & 01.2   & -
        & 01.2   & -
        & 01.2   & - &
        & 01.2   & -
        & 01.2   & -
\\
Full    & 01.3  & 02.3
        & 01.3  & 02.3
        & 01.3  & 02.3 &
        & 01.3  & 02.3
        & 01.3  & 02.3
        & 01.3  & 02.3 
\\
\bottomrule
\end{tabular} 
}
\end{table}

\begin{table}[t]
\centering
\caption{A/B Test on VLOG}
    \begin{tabular}{c@{~~}@{~~}cc@{~~}@{~~}cc@{~~}c@{~~}cc@{~~}@{~~}cc} \toprule
 & 
        \multicolumn{4}{c}{HMR \cite{KanazawaHMR17}} & ~~~~ &
        \multicolumn{4}{c}{CMR \cite{Kolotouros19}} 
\\
Method & 
\multicolumn{2}{c}{$\ge$} & 
\multicolumn{2}{c}{$>$} & &
\multicolumn{2}{c}{$>$} & &
\multicolumn{2}{c}{$\ge$} & 
\multicolumn{2}{c}{$>$} 
\\
$\downarrow \ge \rightarrow$
        & Crop  & Full 
        & Crop  & Full & 
        & Crop  & Full
        & Crop  & Full 
        \\ 
        \midrule
Base    
        & 01.2   & 01.3
        & 01.2   & 01.3 & 
        & 01.2   & 01.3
        & 01.2   & 01.3
\\
Crop    & -     & 02.3
        & -     & 02.3 & 
        & -     & 02.3
        & -     & 02.3
\\
\bottomrule
\end{tabular} 
\end{table}
\end{comment}


